Principal Component Flow Map Learning of PDEs from Incomplete, Limited, and Noisy Data

We present a computational technique for modeling the evolution of dynamical systems in a reduced basis, with a focus on the challenging problem of modeling partially-observed partial differential equations (PDEs) on high-dimensional non-uniform grids. We address limitations of previous work on data-driven flow map learning in the sense that we focus on noisy and limited data to move toward data collection scenarios in real-world applications. Leveraging recent work on modeling PDEs in modal and nodal spaces, we present a neural network structure that is suitable for PDE modeling with noisy and limited data available only on a subset of the state variables or computational domain. In particular, spatial grid-point measurements are reduced using a learned linear transformation, after which the dynamics are learned in this reduced basis before being transformed back out to the nodal space. This approach yields a drastically reduced parameterization of the neural network compared with previous flow map models for nodal space learning. This allows for rapid high-resolution simulations, enabled by smaller training data sets and reduced training times.

==> memory_stuff.tex <==
\subsection{Determining memory length}
The memory length $N_{mem}$ required to adequately represent the relevant dynamics of the system is a question that has not been addressed by the flow map learning literature. It is a challenging, problem-dependent question further complicated by the interaction with the recurrent loss length $N_{rec}$. Additionally, the selection criterion must be a priori. That is, we cannot let a trained model inform our decision. Here, we present a technique to give an estimate of the memory needs.

Let $\Delta t$ be the fixed time-step at which system observations are made, and similar to the above approach for determining an appropriate reduced order dimension, reshape the training trajectories into an $N_{train}N_{full}\times N_{time}$ matrix, call it $B$, where $N_{time}$ is the maximum length less than or equal to all trajectory lengths. Note that the column dimension is in time.

Compute the unique thin QR decomposition of this matrix,
\begin{align}
B = \hat{Q}\hat{R}    
\end{align}
where
\begin{itemize}
\item $\hat{Q}\in\mathbb{R}^{N_{train}N_{full}\times N_{time}}$ has orthonormal columns
\item and $\hat{R}\in\mathbb{R}^{N_{time}\times N_{time}}$ is upper-triangular with non-negative diagonal.
\end{itemize}
Plot the diagonal elements of $\hat{R}$. The size of these elements, and their decay, shows how successive columns of $A$ explain variation within the data across the time dimension. That is, the amount of variation in the span of the first $r$ columns of $A$ (where $r<n$) relative to all the columns. In particular,
\begin{align}
    \hat{R}_{k,k} = \min_{\mathbf{x}\in\mathbb{R}^{k-1}}\left\|A_{:,1:k-1}\mathbf{x}-A_{:,k}\right\|_2
\end{align}
In words, we may say $\hat{R}_{k,k}$ represents the extent to which the $k$-th column of $A$ lies beyond the span of the first $k-1$ columns. We can also look at the relative value $\hat{R}_{k,k}/\|A_{:,k}\|_2$.

We can experiment by how much information is lost if we truncate the QR decomposition after $r$ elements. Similar to the SVD analysis, this shows how much variation in time is explained by the first $r$ observations. %If the values don't decay, this is an indication that the system exhibits a short memory or perhaps is memory-less. If the values decay slowly, the system may require a long memory period.

\begin{figure}[htbp]
	\begin{center}
        \includegraphics[width=.32\textwidth]{./Figures/ex1_memory}
		\includegraphics[width=.32\textwidth]{./Figures/ex2_memory}
        \includegraphics[width=.32\textwidth]{./Figures/ex3_memory}
		\caption{Ex. 2: Determining memory length.}
		\label{fig:ex2_memory}
	\end{center}
\end{figure}
